Metaphorical User Simulators for Evaluating Task-oriented Dialogue Systems

Task-oriented dialogue systems (TDSs) are assessed mainly in an offline setting or through human evaluation. The evaluation is often limited to single-turn or is very time-intensive. As an alternative, user simulators that mimic user behavior allow us to consider a broad set of user goals to generate human-like conversations for simulated evaluation. Employing existing user simulators to evaluate TDSs is challenging as user simulators are primarily designed to optimize dialogue policies for TDSs and have limited evaluation capabilities. Moreover, the evaluation of user simulators is an open challenge. In this work, we propose a metaphorical user simulator for end-to-end TDS evaluation, where we define a simulator to be metaphorical if it simulates user's analogical thinking in interactions with systems. We also propose a tester-based evaluation framework to generate variants, i.e., dialogue systems with different capabilities. Our user simulator constructs a metaphorical user model that assists the simulator in reasoning by referring to prior knowledge when encountering new items. We estimate the quality of simulators by checking the simulated interactions between simulators and variants. Our experiments are conducted using three TDS datasets. The proposed user simulator demonstrates better consistency with manual evaluation than an agenda-based simulator and a seq2seq model on three datasets; our tester framework demonstrates efficiency and has been tested on multiple tasks, such as conversational recommendation and e-commerce dialogues.

==> tables/case-studies.tex <==

\begin{table*}[!t]
\small \centering
\setlength\tabcolsep{4pt}
\caption{Case study} \label{table:outputs2}
\begin{tabular}{@{}rp{15cm}@{}}
\toprule
\textbf{Topic} &{Online shopping}\\
\midrule
\multirow{3}{*}{\textbf{Context}}
& \underline{User2}: I like to shop online, probably a bit too much.\\
& \underline{User1}: Lol me too! \textcolor{red}{What's your favorite online store?}\\
& \underline{User2}: I love to shop on amazon. So you shop online a lot too? Where do you shop? \\
\midrule
\multicolumn{2}{@{}l}{\textbf{Model outputs}}\\
DukeNet &{i shop in amazon . i shop at the amazon . they are an american multinational technology company based in seattle , washington .}\\
KnowledGPT &{i shop online at amazon. it's a great online store. i like to shop at amazon.}\\
KnowExpert &{i shop online at amazon. i like to shop online because i can find the best deals online.}\\
MSDP &{Yes I do . I shop online a lot too . I know that Online shopping is a form of electronic commerce which allows consumers to directly buy goods or services from a seller over the Internet using a web browser .}\\
\textbf{MixCL} &{I do! I like to shop online at \textcolor{Green}{Amazon.com and Barnes \& Noble.} \textcolor{red}{What's your favorite store?}}\\
\midrule
\textbf{Human} &{Amazon as well. I also shop a lot online at Old Navy and Gap. They have great sales.}\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/eval-simulator.tex <==
\begin{table*}[!t]
\centering
\small
\setlength\tabcolsep{2pt}
\caption{Evaluation results of user simulators. Dist denotes for \textsc{Distinct}, Coh. denotes \textsc{Coherence}, and Hum. denotes for \textsc{Human-like}. Boldface indicates the best results in the corresponding metric; significant improvements over the best baseline are marked with * (t-test, $p<0.05$).}
\label{table:simulator}
{%
\begin{tabular}{@{}l  ccccccc  ccccccc  ccccc@{}}

\toprule

{\textbf{Datasets}} 
& \multicolumn{7}{c}{\textbf{MultiWOZ}} 
& \multicolumn{7}{c}{\textbf{ReDial}} 
& \multicolumn{5}{c}{\textbf{JDDC}}\\

\cmidrule(lr){2-8} \cmidrule(lr){9-15}  \cmidrule(lr){16-20}  

{}
& \multicolumn{3}{c}{Test set} 
& \multicolumn{2}{c}{Interaction}
& \multicolumn{2}{c}{Human}
& \multicolumn{3}{c}{Test set} 
& \multicolumn{2}{c}{Interaction}
& \multicolumn{2}{c}{Human}
& \multicolumn{3}{c}{Test set} 
& \multicolumn{1}{c}{Interaction}
& \multicolumn{1}{c}{Human} 
\\
\cmidrule(r){2-4}
\cmidrule(r){5-6}
\cmidrule(r){7-8}
\cmidrule(r){9-11}
\cmidrule(r){12-13}
\cmidrule(r){14-15}
\cmidrule(r){16-18}
\cmidrule(r){19-19}
\cmidrule{20-20}
& F1     & Dist   &  Slot  & Success  & Dist   & Coh.   & Hum.
& F1     & Dist   &  Slot  & Success  & Dist   & Coh.   & Hum.
& F1     & Dist   &  Slot   & Dist   & Hum.
\\ 

\midrule

Agenda~\citep{Schatzmann2007AgendaBasedUS}
& 27.25    &  18.18   & 27.73    & 12.19  & 14.15    & 1.96     &  1.84
& 16.58    &  \textbf{24.36}   & 7.44    & 4.84    & 22.97    & 2.45    &   1.95
& 13.18    &  22.42   & 8.95    &  29.37   & 1.81
\\

AgendaGen~\citep{Shi2019HowTB}
& 34.51    & 16.91    & 24.68 &  32.17   & 13.58    &  2.20   & 1.98   
& 21.06    & 18.81    & 7.15    &  6.78   & \textbf{23.04}    & 2.42    &   2.10 
& 17.32    & 25.36    & 10.53     &  31.49   &   1.97 
\\

SL+Template~\citep{Shi2019HowTB}
& 35.54    & \textbf{20.20}    &  42.02   &  59.78   & 12.74    &  2.20   &   1.75
& 27.83    &  23.27   &  15.07    & 7.30   & 19.26    & 2.64    &    2.30
& 12.91    &  25.28   &  40.55    &  28.74   &     1.86
\\

Seq2seq~\citep{Raffel2020ExploringTL}
& 42.02    &  14.98   & 49.41   &  76.75   &  13.76   & 2.18    &   2.04
& 29.75    &  16.97   & 11.28    & 6.18   &  16.45   &  2.30   &  2.35  
& 23.45    &  21.29   & 37.26     & 23.29    &    2.22
\\


\midrule

\textbf{MetaSim}
& \textbf{44.13}\rlap{*}    & 17.29    & \textbf{57.65}\rlap{*}    & \textbf{80.25}\rlap{*}   & \textbf{15.65}    &   \textbf{2.31}  & \textbf{2.21}  
& \textbf{33.79}\rlap{*}    & 20.43    & \textbf{15.72}\rlap{*}    & \textbf{13.70}\rlap{*}    &  20.97   &  \textbf{2.70}   &  \textbf{2.41}  
& \textbf{23.85}    & \textbf{26.37}\rlap{*}    & \textbf{44.00}\rlap{*}     & \textbf{34.81}\rlap{*}    &    \textbf{2.38}
\\

MetaSim-Metaphor
& 43.31    & 16.83    & 55.27    & 78.96    & 15.32    & 2.25    &   2.13
& 32.59    & 18.94    & 15.21    & 12.74    & 19.36    & 2.66    &    2.35
& 23.42    & 25.41    & 43.65      & 32.65    &  2.31 
\\

MetaSim-Policy
& 43.11    & 14.65    & 49.46    & 71.54    & 14.18    &  2.20   &  2.17
& 33.67    & 15.80    & 13.01    & 12.87    &  17.39   & 2.35    & 2.14
& 22.35    & 20.46    & 39.55    &  30.11   &    2.14
\\

MetaSim-Preference
& 33.84    &  12.71   & \ \ 9.76    &  \ \ 0.93   &  \ \ 5.20    & 1.98    &   1.72
& 32.18    &  14.25   & \ \ 4.35    & 3.43   & \ \ 5.09    & 2.05    &  2.05  
& 18.13    &  19.76   & 22.32    &  \ \ 0.09   &  1.77  
\\
\bottomrule
\end{tabular}
}

\end{table*}


==> tables/policy.tex <==
\begin{table}[!t]
\setlength\tabcolsep{2pt}
\caption{Component evaluation of policy module.}
\label{table:main}
\begin{tabular}{l cccc cc}

\toprule

{\textbf{}} 
& \multicolumn{4}{c}{\textbf{Test set}} 
& \multicolumn{2}{c}{\textbf{Simulator}}\\

\cmidrule(lr){2-5} \cmidrule(lr){6-7}

\textbf{Model} & Inform & Success & BLEU & Combine & Success & Div.\\

\midrule

Baseline & 89.63 & 79.32 & 18.36 & 102.53 & & \\

MetaSim & 89.63 & 79.32 & 18.36 & 102.53 & 78.25 & 16.32 \\
+RL & 89.63 & 79.32 & 18.36 & 102.53 & & \\

\bottomrule
\end{tabular}

\end{table}


==> tables/rl.tex <==
\begin{table}[!t]
\setlength\tabcolsep{2pt}
\caption{Results of System with Continue Training (SCT). }
\label{table:tl}
\begin{tabular}{l cccc cc}

\toprule

{\textbf{}} 
& \multicolumn{4}{c}{\textbf{Test set}} 
& \multicolumn{2}{c}{\textbf{Simulator}}\\

\cmidrule(lr){2-5} \cmidrule(lr){6-7}

\textbf{Model} & Inform & Success & BLEU & Combine & Success & Distinct.\\

\midrule

System & 88.80 & 75.90 & 15.36 & 97.84 & 80.25 & 15.32 \\

\midrule
\textit{10} \% \emph{SCT} & 57.90 & 32.20 & 12.61 & 56.86 & 31.71 & 15.84 \\
% \textit{10} \% &&&&\\
% System & 65.23 & 43.82 & 18.36 & 102.53 & 31.71 & 15.84 \\
% Continue Training &   &   &   &   & & \\

\bottomrule
\end{tabular}

\end{table}

